New Algorithms for Minimizing the Weighted Number of Tardy Jobs On a Single Machine

In this paper we study the classical single machine scheduling problem where the objective is to minimize the total weight of tardy jobs. Our analysis focuses on the case where one or more of three natural parameters is either constant or is taken as a parameter in the sense of parameterized complexity. These three parameters are the number of different due dates, processing times, and weights in our set of input jobs. We show that the problem belongs to the class of fixed parameter tractable (FPT)problems when combining any two of these three parameters. We also show that the problem is polynomial-time solvable when the latter two parameters are constant, complementing Karp's result who showed that the problem is NP-hard already for a single due date.

==> p.tex <==

In this section we show how to modify the algorithm of Section~\ref{section:w} to show that the $1\left\vert {}\right\vert \Sigma w_{j}U_{j} $ problem is also polynomial-time solvable in case $nu_p$ is constant. Let $p_{1},\ldots,p_{nu_p}$ be the set of all processing times in $\mathcal{J}$. Here as well, we start by renumbering the jobs according to the EDD rule, and so $d_{1}\leq d_{2}\leq \ldots\leq d_{n}$. We say that job $J_{j}$ is of type $i$ if its processing time is~$p_i$. A schedule $\pi$ is of \emph{category} $(e_1,\ldots,e_{nu_p}) \in \{1,\ldots,n\}^{nu_w}$, if there are exactly $e_i$ early jobs of type $i$ in $\pi$. The following elimination property holds:
\begin{lemma}
\label{lemma:p1}%
Let $\pi_j^1$ and $\pi_j^2$ be two schedules of the same category for $\mathcal{J}_j$, and let $W_1$ and~$W_2$ denote the total weight of the early jobs in $\pi_j^1$ and $\pi_j^2$, respectively. If $W_1 \geq W_2$, then $\pi_j^1$ dominates $\pi_j^2$.
\end{lemma}

\begin{proof}
First note that the set of early jobs in both two partial schedules has the same total processing time of $\Sigma_{i=1}^{nu_p} p_{i}e_{i}$. Now, consider an optimal extension of $\pi_j^2$ to a complete schedule $\pi^2$. Extend $\pi_j^1$ to a complete schedule $\pi^1$ by setting $\pi^1(J_i) = \pi^2(J_i)$ for $i=j+1,...,n$. The fact that $\Sigma_{i=1}^{nu_p} p_{i}e_{i}$ implies that each of the jobs $J_{j+1},...,J_n$ is completed at the same time in both complete schedules. Let $W'$ be the total weight of the early jobs among jobs $J_{j+1},...,J_n$ in both complete schedules. Then, the total weight of the early jobs in $\pi^2$ is $W_2+W'$ and in $\pi^2$ is $W_1+W'$. The fact that $W_1 \geq W_2$ leads to the conclusion that $\pi_j^1$ indeed dominates $\pi_j^2$.
\end{proof}


Now, let $W_{j}(e_{1},\ldots,e_{nu_p})$ represent the maximum total weight of the early jobs among all schedules of category $(e_1,\ldots,e_{nu_p})$ for job set $\mathcal{J}_j$. In a similar way to what was done in Section~\ref{section:w}, for each job index $j$ and category $(e_1,\ldots,e_{nu_p})$, we maintain a heap $H'_{i,j}(e_1,\ldots,e_{nu_p})$ that contains the weights of $e_i$ early jobs of type $i$. These weights will be kept as large as possible throughout the computation, making sure that indeed we keep the state of maximum weight among all possible states with the same number of early jobs $e_i$ for $i=1,...,nu_p$. Here as well, a standard implementation of $H'_{i,j}(e_1,\ldots,e_{nu_p})$ allows us to insert or remove an element from $H'_{i,j}(e_1,\ldots,e_{nu_p})$ in $O(\lg n)$ time, as well as obtain its \emph{minimum} value $h'_{i,j}(e_1,\ldots,e_{nu_p})$ in $O(1)$ time.
%Note that by construction, our $k$ heaps $H_{i,j}(e_1,\ldots,e_{w_{\#}})$, $1\leq i \leq k$, will correspond to a schedule $\pi_j$ for $\mathcal{J}_j$ of category $(e_1,\ldots,e_{w_{\#}})$ whose total length of the early jobs of type $i$  it will hold that all $k$ heaps $H_{i,j}(e_1,\ldots,e_{w_{\#}})$ for each $i=1,\ldots,w_{\#}$, the for each job index $j$ and category $P_j(e_1,\ldots,e_{w_{\#}})$, there

Our dynamic program computes the values $W_j(e_1,\ldots,e_{nu_p})$ in increasing $j$ and $e_1,\ldots,e_{nu_p}$, using the minimum values of the heaps computed in previous steps. Assume that job $J_j$ is of type~$i$.
We consider two cases:\\



% Furthermore, for each $i=1,\ldots,nu_p$, define the pivot value
%$$
%w_{i,j}(e_1,\ldots,e_{nu_p}) = \max_{\pi_j} \min \{w : w\text{ is the weight of an early job of type } i \text{ in } \pi_j \},
%$$
%where the maximum is taken over all schedules $\pi_j$ of category $(e_1,\ldots,e_{nu_p})$ for $\mathcal{J}_j$ with total weight of early jobs equalling $W_{j}(e_{1},e_{2},\ldots,e_{nu_p})$.

\begin{itemize}
\item \underline{$\sum_{i=1}^{nu_p} p_{i}e_{i} > d_{j}$}: In this case we can only use $J_j$ to replace the least weighted early job of type $i$ (say job $J_l$, $l<j$) in a schedule of the same category for $\mathcal{J}_{j-1}$. Accordingly, we set
$$
W_j(e_1,\ldots,e_{nu_p}) = W_{j-1}(e_1,\ldots,e_{nu_p})+\max\{0,w_j-h'_{i,j-1}(e_1,\ldots,e_{nu_p})\}.
$$
Note that if we replace $J_l$ by $J_j$, then indeed job $J_j$ will be early, as both jobs share the same processing time of $p_i$, and $d_l\leq d_j$.
We then update the set of $k$ heaps corresponding to $W_j(e_1,\ldots,e_{nu_p})$ as follows. We first set $H'_{i_0,j}(e_{1}\ldots,e_{nu_p}) = H'_{i_0,j-1}(e_{1}\ldots,e_{nu_p})$ for all $i_0=1,\ldots,k$. Then, if $w_j > h'_{i,j}(e_{1}\ldots,e_{nu_p})$, we remove $h'_{i,j}(e_{1}\ldots,e_{nu_p})$ from $H'_{i,j}(e_{1}\ldots,e_{nu_p})$, and add $w_j$ instead.

\item \underline{$\sum_{i=1}^{nu_p} p_{i}e_{i} \leq d_{j}$}: In this case, we can also safely add $J_j$ to set of early jobs of the schedule corresponding to $W_{j-1}(e_{1},\dots,e_{i}-1,\dots,e_{nu_p})$. Therefore, we have
$$
W_j(e_1,\ldots,e_{nu_p})= \max
\begin{cases}
W_{j-1}(e_1,\ldots,e_{nu_p})+\max\{0,w_j-h'_{i,j-1}(e_1,\ldots,e_{nu_p})\}, \\
W_{j-1}(e_1,\ldots,e_i-1,\ldots,e_{nu_p})+w_{j}.
\end{cases}
$$
\end{itemize}
%
We implement the above recursion and update the heaps accordingly for all $j\in \{0,\ldots,n\}$ and $e_i\in \{0,\ldots,n_{i,j}\}$, where $
n_{i,j}$ is the number of jobs of type $i$ in $\mathcal{J}_j$. The bases cases for the recursion above are given by
$$
W_0(e_1,\ldots,e_{nu_p})=
\begin{cases}
0 & \text{if }e_{1}=e_{2}=\ldots=e_{nu_p}=0, \\
-\infty & \text{otherwise},
\end{cases}
$$
and the heaps are initialized by $H'_{i,0}(0,\ldots,0)=\emptyset$ for all $i\in \{1,\ldots,nu_p\}$. At the end of the dynamic program, the optimal solution is the one that corresponds to the maximum $W_{n}(e_1,e_2,\ldots,e_{nu_p})$ value, among all those values computed at stage $j=n$. Let $W^{*}_{n}(e_1,e_2,\ldots,e_{nu_p})$ be that maximal value, then the following lemma holds:
\begin{lemma}
$Z^* = \sum_{j=1}^{n} w_j - W^{*}_{n}(e_1,e_2,\ldots,e_{nu_p})$ is the minimum total weighted number of tardy jobs among all schedules for $\mathcal{J}$.
\end{lemma}


Note that running time of our algorithm is dominated by the dynamic program implementation. There are $O(n^{nu_p+1})$ different $W_j(e_1,e_2,\ldots,e_{nu_p})$ values to compute each of which requires $O(1)$ time. Moreover, we update $O(n^{nu_p+1})$ different heaps each of these requires in $O(lgn)$ time. Thus, the running time of the dynamic program implementation is bounded by $O(n^{nu_p+1}lgn)$, and the second part of Theorem~\ref{theorem:poly} holds.


% value computed in the among all states computed at stage $n$.  Let $e_{i}^{\ast }$ be the optimal number of early jobs of type $i$ ($i\in
%\{1,\ldots,nu_p$\})\ such that $Z^{\ast }=\Sigma
%_{i=1}^{nu_p}w_{i}(n_{in}-e_{i}^{\ast })$ is the minimal weighted number of tardy jobs. Then the optimal set of early jobs of
%type $i$ is $E_{in}(e_{1}^{\ast },e_{2}^{\ast },\ldots,e_{nu_p}^{\ast })$ for
%$i\in \{1,\ldots,nu_p\}$. Since there are $O(n^{nu_p})$ state vectors $%
%(e_{1},e_{2},\ldots,e_{nu_p})$ in each stage $j\in \{1,2,\ldots,n\}$, the
%implementation of the recursion requires the calculation of $O(n^{nu_p+1})$
%different $F_{j}(e_{1},e_{2},\ldots,e_{nu_p})$ values, each of which requires
%$O(\log n)$ time due to the need to maintain the lists in an \emph{SWF}
%order. Therefore, the following theorem holds:
%
%\begin{theorem}
%The $1\left\vert {}\right\vert \Sigma w_{j}U_{j}$ problem is solvable in $%
%O(n^{nu_p+1}\log n)$ time$.$
%\end{theorem}
%

